Clustering Hierarchies via a Semi-Parametric Generalized Linear Mixed Model: a statistical significance-based approach

We introduce a novel statistical significance-based approach for clustering hierarchical data using semi-parametric linear mixed-effects models designed for responses with laws in the exponential family (e.g., Poisson and Bernoulli). Within the family of semi-parametric mixed-effects models, a latent clustering structure of the highest-level units can be identified by assuming the random effects to follow a discrete distribution with an unknown number of support points. We achieve this by computing {\alpha}-level confidence regions of the estimated support point and identifying statistically different clusters. At each iteration of a tailored Expectation Maximization algorithm, the two closest estimated support points for which the confidence regions overlap collapse. Unlike the related state-of-the-art methods that rely on arbitrary thresholds to determine the merging of close discrete masses, the proposed approach relies on conventional statistical confidence levels, thereby avoiding the use of discretionary tuning parameters. To demonstrate the effectiveness of our approach, we apply it to data from the Programme for International Student Assessment (PISA - OECD) to cluster countries based on the rate of innumeracy levels in schools. Additionally, a simulation study and comparison with classical parametric and state-of-the-art models are provided and discussed.

==> tables/Sim_Bin_int.tex <==
\label{tab_Ber_int}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)     &   $\hat{\beta}_1$(sd)\\
                  
         
\midrule
\midrule 

              &2        & 0.002        & 0.000 (-)        & [0.70 (-), 0.30 (-)]                                 &  [2.21 (-), -8.13 (-)] &  -4.81 (-) \\
$\alpha=0.01$ &\bftab 3 & \bftab 0.980 & \bftab 0.002 (0.01)& \bftab[0.20 (0.16), 0.50 (0.16), 0.30 (0.00)]        &  \bftab [5.13 (0.62), 2.05 (0.28), -9.93 (1.01)] & \bftab-6.13 (0.62)   \\
              &4        & 0.018        & 0.010 (0.01)      & [0.17 (0.47), 0.29 (1.29), 0.24 (1.71), 0.30 (0.00)] &  [5.78 (0.33), 3.25 (0.60), 1.28 (0.71), -10.42 (0.80)]& -6.62 (0.62)  \\

\midrule
              &2        & 0.002       & 0.000 (-)         & [0.70 (-), 0.30 (-)]                                 & [2.54 (-), -8.76 (-)] &  -5.59 (-) \\
$\alpha=0.05$ &\bftab 3 &\bftab 0.966 & \bftab 0.001 (0.01) & \bftab[0.20 (0.14), 0.50 (0.14), 0.30 (0.00)]        & \bftab [5.15 (0.62), 2.04 (0.28), -9.93 (1.05)] & \bftab-6.14 (0.63)  \\
              &4        & 0.028       & 0.041 (0.03)       & [0.18 (0.41), 0.24 (1.34), 0.29 (1.39), 0.29 (0.26)] & [5.65 (0.52), 3.20 (0.55), 0.91 (2.94), -10.67 (1.03)]& -6.66 (0.69) \\
\midrule      
              
              &2        &  -          &  -                  &           -                                          & - &  -  \\
$\alpha=0.10$ &\bftab 3 &\bftab 0.916 & \bftab 0.001 (0.01) & \bftab [0.20 (0.10), 0.50 (0.10), 0.30 (0.00)]       & \bftab [5.14 (0.59), 2.05 (0.29), -9.98 (0.99)] & \bftab-6.16 (0.59)  \\
              &4        &  0.080      & 0.045 (0.04)       & [0.18 (0.42), 0.30 (1.48), 0.25 (1.48), 0.27 (0.55)] & [5.63 (0.69), 2.93 (0.81), -0.76 (4.45), -10.62 (1.23)]& -6.50 (0.71) \\

\midrule
\midrule

         &2       &0.004      &    0.000 (0.00)  &      [0.70 (0.00), 0.30 (0.00)]                    &[2.42 (0.10), -9.20 (1.23)] &  -5.59 (0.97) \\
$t=0.50$ &\bftab 3&\bftab0.812&\bftab 0.001 (0.00)&\bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]       &\bftab [5.14 (0.59), 2.05 (0.27), -10.03 (0.97)] &\bftab-6.19 (0.61) \\
         &4       &0.174      &    0.074 (0.06)   &[0.18 (0.42), 0.33 (1.71), 0.25 (1.60), 0.24 (0.81)]&[5.54 (0.76), 2.88 (1.07), -2.78 (5.54), -10.66 (1.29)]& -6.35 (0.69) \\
\midrule

         &2       &0.008      &    0.000 (0.00)  &      [0.70 (0.00), 0.30 (0.00)]                    &[2.35 (0.15), -8.66 (0.63)] &  -5.05 (0.28) \\
$t=0.75$ &\bftab 3&\bftab0.858&\bftab 0.002 (0.01)&\bftab[0.20 (0.27), 0.50 (0.19), 0.30 (0.10)]       &\bftab [5.09 (0.59), 2.02 (0.54), -9.92 (0.99)] &\bftab-6.14 (0.60) \\
         &4       &0.130      &    0.057 (0.02)   &[0.18 (0.41), 0.39 (1.62), 0.22 (1.5), 0.22 (0.81)]&[5.40 (0.70), 2.61 (0.92), -4.53 (5.39), -10.73 (1.13)]& -6.28 (0.67) \\         

\midrule 

         &2       &0.016      &    0.000 (0.00)  &      [0.70 (0.00), 0.30 (0.00)]                    &[2.36 (0.19), -8.44 (0.60)] &  -5.10 (0.39) \\
$t=1.00$ &\bftab 3&\bftab0.876&\bftab 0.002 (0.01)&\bftab[0.20 (0.27), 0.50 (0.19), 0.30 (0.10)]       &\bftab [5.10 (0.64), 2.00 (0.60), -9.94 (1.02)] &\bftab-6.13 (0.65) \\
         &4       &0.108      &    0.051 (0.03)   &[0.19 (0.37), 0.43 (1.38), 0.19 (1.26), 0.20 (0.79)]&[5.34 (0.73), 2.41 (0.93), -5.93 (4.96), -10.68 (1.26)]& -6.23 (0.65) \\         

\midrule

         &2       &0.040      &    0.000 (0.00)  &      [0.70 (0.00), 0.30 (0.00)]                    &[2.41 (0.21), -8.30 (0.81)] &  -5.03 (0.50) \\
$t=1.25$ &\bftab 3&\bftab0.922&\bftab 0.001 (0.01)&\bftab[0.20 (0.27), 0.50 (0.23), 0.30 (0.05)]       &\bftab [5.14 (0.64), 2.01 (0.50), -9.92 (0.97)] &\bftab-6.13 (0.59) \\
         &4       &0.038      &    0.039 (0.03)   &[0.18 (0.36), 0.43 (1.45), 0.23 (1.22), 0.15 (0.82)]&[5.88 (0.67), 2.60 (0.97), -7.56 (5.10), -12.03 (1.66)]& -6.64 (0.70) \\         

\midrule

         &2       &0.064      &    0.000 (0.00)  &      [0.70 (0.00), 0.30 (0.00)]                    &[2.35 (0.24), -8.16 (0.74)] &  -4.95 (0.50) \\
$t=1.50$ &\bftab 3&\bftab0.900&\bftab 0.001 (0.01)&\bftab[0.20 (0.20), 0.50 (0.20), 0.30 (0.00)]       &\bftab [5.13 (0.59), 2.03 (0.27), -9.95 (1.03)] &\bftab-6.14 (0.61) \\
         &4       &0.036      &    0.050 (0.03)   &[0.19 (0.31), 0.46 (1.11), 0.19 (1.03), 0.16 (0.68)]&[5.46 (0.59), 2.41 (0.57), -8.30 (3.76), -11.64 (1.21)]& -6.52 (0.59) \\    
         
   
\midrule
\midrule 

TV       & &     &  & [0.2, 0.5, 0.3]  &   $[5,2,-10]$          &   $-6$            \\
\vspace{-0.35cm}

==> tables/Sim_Bin_int2.tex <==
\label{tab_Ber_int2}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)     &   $\hat{\beta}_1$(sd)&    $\hat{\beta}_2$(sd)\\
             
\midrule
\midrule 

               &2       & 0.008      & 0.000 (0.00)      & [0.70 (0.00), 0.30 (0.00)]                         &[2.46 (0.24), -8.98 (1.06)] & -5.38 (0.50) & 2.79 (0.31)\\
$\alpha=0.01$  &\bftab 3&\bftab 0.970&\bftab 0.002 (0.01)&\bftab [0.20 (0.16), 0.50 (0.16), 0.30 (0.00)]      &\bftab [5.16 (0.63), 2.05 (0.29), -10.23 (1.09)] & \bftab -6.20 (0.64) &  \bftab 3.11 (0.36)\\
               &4       & 0.022      & 0.024 (0.02)      &[0.19 (0.29), 0.40 (0.85), 0.17 (0.62), 0.24 (0.88)]&[5.19 (0.52), 2.58 (0.42), -2.90 (5.22), -11.30 (1.17)] & -6.34 (0.48) & 3.14 (0.30)\\
               
\midrule                
               &2       &  -          & -                 & -                                                  & -  & -  & -  \\
$\alpha=0.05$  &\bftab 3& \bftab 0.952&\bftab 0.002 (0.01)& \bftab [0.20 (0.22), 0.50 (0.22), 0.30 (0.00)]     &[5.17 (0.63), 2.05 (0.30), -10.16 (1.03)] & -6.19 (0.62) & 3.10 (0.36)\\
               &4       &  0.048      &0.032 (0.03)       &[0.19 (0.28), 0.38 (1.30), 0.18 (1.00), 0.25 (0.71)]&[5.38 (0.65), 2.56 (0.58), -2.20 (5.03), -10.92 (1.39)] & -6.41 (0.66) & 3.13 (0.36)\\

\midrule                
               &2       & 0.004      &  0.000 (0.00)     & [0.70 (0.00), 0.30 (0.00)]                         &[2.72 (0.36), -8.83 (1.15)] & -5.33 (0.79) & 2.29 (0.11)\\
$\alpha=0.10$  &\bftab 3&\bftab 0.906&\bftab 0.002 (0.01)& \bftab [0.20 (0.12), 0.50 (0.12), 0.30 (0.00)]     &\bftab [5.15 (0.62), 2.06 (0.29), -10.12 (1.06)] & \bftab -6.19 (0.62) & 3.06 (0.35)\\
               &4       & 0.080      &  0.039 (0.03)     &[0.19 (0.33), 0.38 (1.44), 0.20 (1.32), 0.23 (0.85)]&[5.36 (0.83), 2.67 (0.88), -3.02 (5.27), -10.9 (1.04)] & -6.35 (0.51) & 3.17 (0.26)\\

\midrule 
\midrule  

         &2        &          - & -                 & -  & - & - & - \\
$t=0.50$ &\bftab 3 &\bftab 0.780&\bftab 0.002 (0.01)& \bftab [0.20 (0.40), 0.50 (0.34), 0.30 (0.07)] & \bftab [5.14 (0.66), 2.00 (0.72), -10.22 (1.16)] & \bftab -6.18 (0.68) & \bftab 3.09 (0.35)\\
         &4&         0.196      &0.078 (0.05)       & [0.18 (0.4), 0.33 (1.69), 0.26 (1.43)]  & [5.53 (0.82), 2.82 (1.05), -2.91 (5.55), -10.90 (1.20)] & -6.44 (0.63) & 3.20 (0.37)\\
         
\midrule

         &2&     0.008          & 0.000 (0.00)        & [0.70 (0.00), 0.30 (0.00)]  & [2.36 (0.11), -8.42 (0.30)] & -5.05 (0.30) & 2.55 (0.37) \\
$t=0.75$ &\bftab 3 &\bftab 0.824& \bftab 0.003 (0.01) & \bftab [0.20 (0.18), 0.50 (0.18), 0.30 (0.00)] & \bftab [5.09 (0.65), 2.02 (0.30), -9.99 (1.03)] & \bftab -6.11 (0.63) & \bftab 3.03 (0.32)\\
         &4&     0.154          & 0.053 (0.04)        & [0.18 (0.41), 0.37 (1.65), 0.24 (1.46), 0.21 (0.83)]  & [5.33 (0.71), 2.61 (1.00), -4.52 (5.44), -10.72 (1.19)] & -6.14 (0.65) & 3.07 (0.33)\\
         
\midrule
         &2&     0.010          &0.000 (0.00) & [0.70 (0.00), 0.30 (0.00)]  & [2.56 (0.19), -8.47 (0.50)] & -5.09 (0.37) & 2.45 (0.34) \\
$t=1.00$ &\bftab 3 &\bftab 0.880&\bftab 0.002 (0.01) & \bftab [0.20 (0.18), 0.50 (0.18), 0.30 (0.00)] & \bftab [5.16 (0.61), 2.06 (0.31), -10.17 (1.12)] & \bftab -6.19 (0.68) & \bftab 3.10 (0.37)\\
         &4&     0.110          &0.064 (0.04) & [0.20 (0.36), 0.44 (1.19), 0.16 (1.00), 0.19 (0.70)]  & [5.29 (0.69), 2.25 (0.56), -7.17 (4.44), -11.23 (0.87)] & -6.43 (0.54) & 3.21 (0.30)\\

\midrule
         &2&     0.044          & 0.000 (0.00) & [0.70 (0.00), 0.30 (0.00)] & [2.38 (0.17), -8.23 (0.59)] & -4.84 (0.38) & 2.41 (0.26)\\
$t=1.25$ &\bftab 3 &\bftab 0.910& \bftab 0.002 (0.01) & \bftab [0.20 (0.24), 0.50 (0.24), 0.30 (0.00)] & \bftab [5.22 (0.70), 2.04 (0.29), -10.16 (1.06)] & \bftab -6.19 (0.62) & \bftab 3.09 (0.36)\\
         &4&     0.046          & 0.049 (0.03) & [0.20 (0.00), 0.50 (0.00), 0.15 (0.50), 0.15 (0.50)] & [5.45 (0.62), 2.20 (0.28), -9.61 (0.96), -11.95 (1.40)] & -6.60 (0.60) & 3.33 (0.32)\\

\midrule
         &2&     0.064          & 0.000 (0.00) & [0.70 (0.00), 0.30 (0.00) & [2.40 (0.24), -8.38 (0.72)] & -5.05 (0.48) & 2.55 (0.29)\\
$t=1.50$ &\bftab 3 &\bftab 0.898& \bftab 0.002 (0.01) & \bftab [0.20 (0.18), 0.50 (0.18), 0.30 (0.00)] & \bftab [5.25 (0.66), 2.09 (0.31), -10.40 (1.22)] & \bftab -6.30 (0.70) & \bftab 3.15 (0.41)\\
         &4&     0.038          & 0.046 (0.02) & [0.19 (0.31), 0.49 (0.51), 0.17 (0.57), 0.15 (0.60)] & [5.46 (0.70), 2.26 (0.25), -9.56 (3.11), -12.47 (1.99)] & -6.58 (0.80) & 3.25 (0.47)\\


\midrule               
\midrule 


TV       & &     &  & [0.2,0.5,0.3]  &   $[5,2,-10]$          &   $-6$          &    $3$            \\
\vspace{-0.35cm}

==> tables/Sim_Bin_intslope.tex <==
\label{tab_Ber_intsl}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)  &$\hat{c}_2$(sd)    &   $\hat{\beta}_1$(sd)\\
                %ran_var = FALSE, ran_int = TRUE
\midrule    
\midrule

             &2      & 0.016	    &0.000 (0.00)      &[0.70 (0.00), 0.30 (0.00)]                           &[2.14 (0.11), -7.86 (0.49)] & [4.79 (0.26), -0.09 (0.53)] & -4.68 (0.26)\\
$\alpha=0.01$&\bftab3&\bftab0.664&\bftab0.005 (0.02)&\bftab [0.21 (0.56), 0.49 (0.41), 0.3 (0.19)]    &\bftab [5.24 (0.93), 2.02 (0.98), -10.22 (1.20)]& \bftab [10.57 (1.73), 5.22 (0.82), -0.04 (0.54)] & \bftab -6.28 (0.73)\\
             &4      & 0.268	    &0.054 (0.04)      &[0.19 (0.31), 0.40 (1.48), 0.20 (1.17), 0.2 (0.88)]&[5.56 (1.13), 2.49 (0.78), -5.29 (5.85), -10.99 (1.76)]& [11.04 (1.95), 5.64 (1.54), 2.22 (2.49), 0.14 (1.41)] & -6.41 (0.88)\\
             
\midrule   

             &2      & 0.032	    &0.000 (0.00)      &[0.70 (0.00), 0.30 (0.00)] & [2.25 (0.28), -8.15 (0.66)]& [5.02 (0.83), 0.11 (0.50)] & -5.02 (0.52)\\
$\alpha=0.05$&\bftab3&\bftab0.602&\bftab0.003 (0.01)&\bftab [0.20 (0.48), 0.50 (0.39), 0.3 (0.13)] & \bftab [5.30 (0.96), 2.08 (0.83), -10.37 (1.28)]& \bftab [10.71 (1.89), 5.27 (0.80), -0.02 (0.48)] & \bftab -6.41 (0.82)\\
             &4      & 0.316	    &0.061 (0.06)      &[0.20 (0.18), 0.38 (1.58), 0.21 (1.14), 0.21 (0.9)] & [5.44 (0.94), 2.40  (0.64), -4.57 (5.94), -10.99 (1.40)]& [10.92 (1.41), 5.69 (1.53), 2.51 (2.91), 0.08 (1.19)] & -6.53 (0.72)\\
             
\midrule

             &2      & 0.002	    &0.000 (0.00)      &[0.70 (0.00), 0.30 (0.00)] & [2.11 (0.28), -8.14 (0.93)] & [4.72 (0.41), -0.16 (0.23)] & -4.92 (0.58)\\
$\alpha=0.10$&\bftab3&\bftab0.584&\bftab0.003 (0.01)&
\bftab [0.20 (0.20), 0.50 (0.20), 0.30 (0.00)] &\bftab [5.33 (0.90), 2.14 (0.36), -10.39 (1.25)] & \bftab [10.62 (1.59), 5.36 (0.69), -0.07 (0.53)] & \bftab -6.40 (0.77)\\
             &4      & 0.332	    &0.063 (0.05)      &[0.19 (0.29), 0.39 (1.51), 0.21 (1.18), 0.21 (0.89)] &[5.56 (1.04), 2.53 (0.78), -4.69 (5.87), -10.95 (1.37)] & [10.99 (1.73), 5.73 (1.31), 2.31 (2.92), 0.09 (1.34)] & -6.51 (0.67)\\

\midrule               
\midrule  
 
         &2       &0.014       &0.000 (0.00)       & [0.70 (0.00), 0.30 (0.00)] & [2.10 (0.18), -8.01 (0.76)] & [4.89 (0.37), 0.03 (0.45)] & -4.86 (0.52)\\
$t=0.50$ &\bftab 3&\bftab 0.548&\bftab 0.003 (0.01)& \bftab [0.20 (0.13), 0.50 (0.13), 0.30 (0.00)] & \bftab [5.25 (0.75), 2.09 (0.32), -10.11 (1.07)] & \bftab [10.48 (1.34), 5.19 (0.62), -0.01 (0.52)] & \bftab -6.24 (0.69)\\
         &4       &0.358       &0.063 (0.06)       & [0.19 (0.32), 0.35 (1.76), 0.24 (1.33), 0.22 (0.83)] & [5.65 (1.10), 2.58 (0.79), -4.56 (6.10), -10.97 (1.73)] & [11.13 (1.82), 5.70 (1.67), 2.55 (2.79), -0.08 (1.33)] & -6.48 (0.96)\\
         
\midrule

         &2       &0.022       &0.000 (0.00)       & [0.70 (0.00), 0.30 (0.00)]  &[2.01 (0.29), -7.71 (0.52)] &[4.72 (0.33), -0.09 (0.28) & -4.56 (0.49)\\
$t=0.75$ &\bftab 3&\bftab 0.572&\bftab 0.001 (0.00)& \bftab [0.20 (0.17), 0.50 (0.17), 0.30 (0.00)]  &\bftab [5.37 (0.83), 2.09 (0.32), -10.28 (1.18)]& \bftab [10.82 (1.60), 5.28 (0.62), 0.01 (0.49)]& \bftab -6.36 (0.74)\\
         &4       &0.346       &0.051 (0.04)       & [0.19 (0.33), 0.39 (1.66), 0.22 (1.29), 0.20 (0.86)]  &[5.68 (0.99), 2.63 (0.97), -5.43 (5.82), -11.15 (1.52)] &[11.11 (2.03), 6.03 (1.88), 2.11 (2.87), -0.13 (1.30)] & -6.55 (0.74)\\
\midrule

          &2       &0.005      &0.000 (0.00)       & [0.70 (0.00), 0.30 (0.00)] & [2.16 (0.27), -8.56 (0.94)] & [5.14 (0.60), -0.06 (0.44)] & -5.19 (0.58)\\
$t=1.00$  &\bftab 3&\bftab 0.700&\bftab 0.003 (0.01)& \bftab [0.21 (0.66), 0.49 (0.48), 0.30 (0.21)] &\bftab [5.16 (0.91), 1.90 (1.40), -10.17 (1.15)] & \bftab [10.40 (1.64), 5.16 (0.92), 0.01 (0.52)] & \bftab -6.27 (0.72)\\
          &4       &0.232       &0.055 (0.04)       & [0.19 (0.28), 0.39 (1.56), 0.20 (1.17), 0.21 (0.83)] &[5.71 (1.17), 2.47 (0.80), -5.21 (5.84), -11.05 (1.23)] & [11.36 (2.20), 5.86 (1.65), 2.13 (2.74), 0.01 (1.28)] & -6.54 (0.76)\\

\midrule


         &2       &0.076       &0.000 (0.00)       & [0.70 (0.00), 0.30 (0.00)]  &[2.14 (0.27), -8.22 (0.61)] & [4.85 (0.38), -0.06 (0.48)] & -4.96 (0.36)\\
$t=1.25$ &\bftab 3&\bftab 0.708&\bftab 0.004 (0.01)& \bftab [0.21 (0.75), 0.49 (0.59), 0.30 (0.20)]  &\bftab [5.26 (0.96), 1.92 (1.38), -10.25 (1.19)] & \bftab [10.46 (1.68), 5.15 (0.95), 0.03 (0.47)] & \bftab -6.31 (0.72)\\
         &4       &0.202       &0.037 (0.03)       & [0.19 (0.41), 0.37 (1.69), 0.23 (1.38), 0.21 (0.87)]  &[5.80 (1.28), 2.70 (1.06), -4.81 (5.94), -11.22 (1.44)] & [11.52 (2.35), 6.14 (2.14), 2.45 (2.89), 0.30 (1.40)] & -6.56 (0.79)\\
\midrule

         &2       &0.126       &0.000 (0.00)       & [0.70 (0.00), 0.30 (0.00)]  &[2.08 (0.25), -7.98 (0.85)] &[4.80 (0.48), -0.01 (0.39)] & -4.75 (0.49)\\
$t=1.50$ &\bftab 3&\bftab 0.746&\bftab 0.003 (0.01)& \bftab [0.21 (0.85), 0.49 (0.68), 0.30 (0.23)]  &\bftab [5.24 (1.01), 1.83 (1.64), -10.18 (1.19)] & \bftab [10.56 (1.98), 5.12 (0.96), -0.04 (0.62)] & \bftab -6.26 (0.73)\\
         &4       &0.114       &0.038 (0.03)       & [0.20 (0.86), 0.38 (1.67), 0.22 (1.39), 0.20 (0.85)]  & [5.79 (1.38), 2.65 (1.15), -5.48 (5.69), -11.02 (1.34)] & [11.15 (2.13), 6.34 (2.57), 1.86 (3.04), 0.24 (1.51)] & -6.49 (0.60)\\
        

\midrule  
\midrule                 
                


TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \;]$  &  $[\; 5, \;2, \; -10 \;] $  & $[\; 10, \;5, \; 0 \;] $       &   $-6$              \\
\vspace{-0.35cm}

==> tables/Sim_Bin_intslope2.tex <==
\label{tab_Ber_intsl2}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)  &$\hat{c}_2$(sd)    &   $\hat{\beta}_1$(sd)&    $\hat{\beta}_2$(sd)\\
                %ran_var = FALSE, ran_int = TRUE
\midrule    
\midrule  

         &2       &       0.012 &       0.000 (0.00)&[0.70 (0.00), 0.30 (0.00)]&[2.11 (0.27), -8.45 (1.06)] & [4.79 (0.80), 0.21 (0.27)] & -4.96 (0.64) & 2.44 (0.38)\\
$t=0.50$ &\bftab 3&\bftab 0.508 &\bftab 0.002 (0.01)&\bftab[0.21 (0.46), 0.50 (0.29), 0.30 (0.18)]&\bftab [5.28 (0.92), 1.99 (0.95), -10.47 (1.34)] & \bftab [10.56 (1.64), 5.19 (0.84), 0.01 (0.52)] & \bftab -6.33 (0.82) & \bftab 3.17 (0.43)\\
         &4       &       0.380 &       0.064 (0.05)&[0.19 (0.29), 0.39 (1.51), 0.20 (1.20), 0.21 (0.86)]&[5.49 (0.92), 2.49 (0.75), -4.96 (5.86), -11.12 (1.51)] & [10.97 (1.60), 5.74 (1.51), 2.37 (2.76), -0.11 (0.97)] & -6.47 (0.80) & 3.24 (0.44)\\

\midrule      

         &2       &       0.024 &       0.000 (0.00)&[0.70 (0.00), 0.30 (0.00)]&[2.09 (0.33), -8.07 (0.70)] & [4.67 (0.49), -0.05 (0.25)] & -4.79 (0.42) & 2.41 (0.20)\\
$t=0.75$ &\bftab 3&\bftab 0.582 &\bftab 0.001 (0.00)&\bftab[0.21 (0.55), 0.49 (0.49), 0.30 (0.08)]&\bftab [5.31 (0.88), 2.10 (0.81), -10.55 (1.35)] & \bftab [10.65 (1.70), 5.32 (0.83), -0.02 (0.47)] & \bftab -6.44 (0.85) & \bftab 3.20 (0.45)\\
         &4       &       0.334 &       0.062 (0.05)&[0.19 (0.32), 0.37 (1.59), 0.22 (1.18), 0.21 (0.89)]&[5.60 (0.93), 2.53 (0.72), -4.69 (6.10), -11.35 (1.68)] & [11.20 (1.48), 5.95 (1.60), 2.56 (2.88), 0.01 (1.21)] & -6.62 (0.80) & 3.31 (0.45)\\
         
\midrule   

         &2       &       0.064 &       0.000 (0.00)&[0.70 (0.00), 0.30 (0.00)]& [2.01 (0.26), -8.34 (0.78)] & [4.76 (0.48), -0.15 (0.34)] & -4.81 (0.45) & 2.46 (0.24)\\
$t=1.00$ &\bftab 3&\bftab 0.626 &\bftab 0.001 (0.00)&\bftab[0.21 (0.66), 0.49 (0.51), 0.30 (0.20)]&\bftab [5.24 (1.10), 1.97 (1.17), -10.35 (1.26)] & \bftab [10.57 (2.25), 5.15 (0.90), 0.00 (0.51)] & \bftab -6.26 (0.80) & \bftab 3.14 (0.44)\\
         &4       &       0.262 &       0.062 (0.05)&[0.19 (0.30), 0.40 (1.46), 0.20 (1.16), 0.20 (0.85)]& [5.57 (0.90), 2.54 (0.86), -5.74 (5.94), -11.51 (1.59)] & [11.05 (1.80), 5.82 (1.51), 2.05 (2.78), -0.08 (1.38)] & -6.61 (0.83) & 3.32 (0.44)\\

\midrule  

         &2       &       0.064 &       0.000 (0.00)&[0.70 (0.00), 0.30 (0.00)]&[2.09 (0.26), -8.06 (0.63)] & [4.82 (0.45), 0.02 (0.39)] & -4.77 (0.42) & 2.37 (0.25)\\
$t=1.25$ &\bftab 3&\bftab 0.724 &\bftab 0.003 (0.01)&\bftab[0.21 (0.66), 0.49 (0.46), 0.30 (0.22)]&\bftab [5.30 (1.00), 1.94 (1.30), -10.37 (1.25)] & \bftab [10.61 (1.72), 5.16 (0.91), -0.06 (0.51)] & \bftab -6.29 (0.78) & \bftab 3.15 (0.41)\\
         &4       &       0.208 &       0.042 (0.04)&[0.18 (0.36), 0.40 (1.53), 0.21 (1.29), 0.20 (0.85)]&[5.90 (1.43), 2.63 (0.93), -5.72 (6.10), -11.61 (1.74)] & [11.54 (2.36), 6.21 (1.86), 2.07 (2.72), -0.08 (1.29)] & -6.64 (0.90) & 3.29 (0.48)\\

\midrule  

         &2       &       0.112 &       0.000 (0.00)&[0.70 (0.00), 0.30 (0.00)]&[2.13 (0.33), -8.22 (0.85)] & [4.89 (0.53), -0.03 (0.41)] & -4.86 (0.52) & 2.42 (0.30)\\
$t=1.50$ &\bftab 3&\bftab 0.770 &\bftab 0.002 (0.01)&\bftab[0.21 (0.68), 0.49 (0.49), 0.30 (0.22)]& \bftab [5.32 (0.98), 1.92 (1.36), -10.51 (1.36)] & \bftab [10.66 (1.80), 5.19 (1.04), 0.00 (0.48)] & \bftab -6.36 (0.85) & \bftab 3.18 (0.47)\\
         &4       &       0.110 &       0.041 (0.03)&[0.18 (0.37), 0.40 (1.51), 0.22 (1.28), 0.20 (0.88)]& [5.75 (1.00), 2.64 (1.07), -5.77 (5.95), -11.53 (1.65)] & [11.36 (2.00), 6.12 (1.76), 1.89 (2.90), 0.10 (1.72)] & -6.47 (0.68) & 3.24 (0.33)\\

\midrule                 
\midrule    

               &2&  & &   &  &  &     &    \\
$\alpha=0.01$  &\bftab 3&n &n& n & n& n&   n &   n\\
               &4&  & &   &  &  &     &    \\
\midrule               
               &2&  & &   &  &  &     &    \\
$\alpha=0.05$  &\bftab 3&n &n& n & n& n&   n &   n\\
               &4&  & &   &  &  &     &    \\

\midrule  
               &2&  & &   &  &  &     &    \\
$\alpha=0.10$  &\bftab 3&n &n& n & n& n&   n &   n\\
               &4&  & &   &  &  &     &    \\


\midrule                 
\midrule   

TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \;]$  &  $[\; 5, \;2, \; -10 \;] $  & $[\; 10, \;5, \; 0 \;] $       &   $-6$          &    $3$            \\
\vspace{-0.35cm}

==> tables/Sim_Bin_slope.tex <==
\label{tab_Ber_sl}
        &  N clusters  & Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)    & $\hat{\beta}_1$(sd)  &  $\hat{\beta}_2$(sd)\\
                %ran_var = FALSE, ran_int = TRUE
\midrule
\midrule

              &2       & -         & -                & -                                                  &   -                                         & - & -  \\
$\alpha=0.01$ &\bftab 3&\bftab0.986&\bftab0.008 (0.02)&\bftab[0.20 (0.16), 0.50 (0.25), 0.30 (0.19)]       &\bftab[10.51 (1.61), 5.25 (0.77), 0.01 (0.50)]&\bftab10.49 (1.47)&\bftab-6.38 (0.95)   \\
              &4       &0.014      &0.038 (0.04)      &[0.20 (0.00), 0.39 (1.25), 0.20 (0.76), 0.21 (0.64)]&[12.79 (2.72), 6.76 (0.94), 3.24 (0.95), -0.96 (1.20)]&12.25 (2.21) & -7.56 (1.29)    \\
         
\midrule
              &2       &0.002      &0.000 (-)         &[0.70 (0.00), 0.30 (0.00)]                          &[6.35 (-), -0.25 (-)]&10.87 (-)&-6.65 (-)   \\
$\alpha=0.05$ &\bftab 3&\bftab0.920&\bftab0.006 (0.02)&\bftab[0.20 (0.13), 0.50 (0.17), 0.30 (0.14)]       &\bftab[10.46 (1.64), 5.19 (0.83), 0.06 (0.55)]&\bftab10.36 (1.53)&\bftab-6.31 (0.97)   \\
              &4       &0.070      &0.065 (0.05)      &[0.19 (0.28), 0.35 (1.46), 0.23 (1.26), 0.22 (0.83)]&[11.40 (1.93), 6.45 (1.45), 3.27 (1.84), -0.61 (1.16)]&11.16 (1.76) & -6.82 (1.14)    \\

\midrule
              &2       &0.004      &0.000 (0.00)      &[0.70 (0.00), 0.30 (0.00)]                          &[4.78 (0.42), -0.03 (0.17)]&7.39 (0.54)&-4.29 (0.46)\\
$\alpha=0.10$ &\bftab 3&\bftab0.830&\bftab0.005 (0.01)&\bftab[0.20 (0.11), 0.50 (0.15), 0.30 (0.11)]       &\bftab[10.45 (1.50), 5.20 (0.77), -0.02 (0.51)]&\bftab10.38 (1.38)&\bftab-6.32 (0.91)   \\
              &4       &0.158      &0.066 (0.05)      &[0.19 (0.28), 0.34 (1.46), 0.22 (1.21), 0.25 (0.76)]&[11.43 (1.94), 6.47 (1.54), 3.44 (1.79), -0.51 (1.03)]&11.23 (1.92) & -6.81 (1.18)    \\

\midrule 
\midrule

         &2       & 0.022      & 0.001 (0.00)        &[0.70 (0.00), 0.30 (0.00)]                          & [4.49 (0.57), 0.08 (0.44)] & 7.21 (0.93) & -4.22 (0.59) \\
$t=0.50$ &\bftab 3&\bftab 0.704&\bftab 0.005 (0.01)  &\bftab [0.20 (0.09), 0.50 (0.16), 0.30 (0.13)]      &\bftab [10.58 (1.72), 5.28 (0.87), -0.01 (0.54) ]& \bftab 10.57 (1.56) & \bftab   -6.44 (0.98)  \\
         &4       & 0.230      & 0.100 (0.07)        &[0.19 (0.29), 0.36 (1.63), 0.22 (1.34), 0.23 (0.82)]& [10.91 (1.72), 6.06 (1.36), 3.06 (1.91), -0.50 (0.87)] & 10.73 (1.58) & -6.56 (1.05)  \\
\midrule

         &2       & 0.058      & 0.005 (0.01)      &[0.68 (0.93), 0.32 (0.93)]                          & [4.57 (0.55), 0.22 (0.45)] & 7.13 (0.68) & -4.21 (0.40) \\
$t=0.75$ &\bftab 3&\bftab 0.754&\bftab 0.005 (0.02)&\bftab [0.20 (0.41), 0.50 (0.31), 0.30 (0.26)]      & \bftab [10.45	(1.67), 5.22 (0.89), -0.01 (0.57)] & \bftab 10.48 (1.49) & \bftab -6.39 (0.96) \\
         &4       & 0.174      & 0.099 (0.06)      &[0.20 (0.19), 0.38 (1.39), 0.20 (0.99), 0.22 (0.84)]& [10.84 (1.81), 5.81 (1.50), 2.73 (2.15), -0.74 (0.83)] & 10.79 (1.90) & -6.58 (1.20)\\
\midrule

          &2       & 0.178      & 0.006 (0.02)       &[0.63 (1.57), 0.37 (1.57)]                          &[4.93 (1.03), 0.34 (0.78)] & 7.33 (0.85) & -4.38 (0.59)\\
$t=1.00$  &\bftab 3&\bftab 0.760&\bftab 0.007 (0.02) &\bftab [0.21 (0.71), 0.49 (0.54), 0.30 (0.28)]      &\bftab [10.29 (1.81), 5.09 (1.04), -0.03 (0.54)] & \bftab 10.33 (1.59) &\bftab -6.29 (1.04)\\
          &4       & 0.060      &  0.088 (0.05)      &[0.20 (0.18), 0.40 (1.38), 0.21 (0.89), 0.19 (0.85)]&[11.46 (1.79), 6.09 (1.06), 2.30 (2.22), -1.33 (1.15)] & 11.48 (1.66) & -7.00 (1.04)\\

\midrule

         &2       & 0.368      &  0.007 (0.02)      &[0.66 (1.29), 0.34 (1.29)]                          &[4.78 (1.01), 0.28 (0.75)] & 7.27 (0.81) & -4.32 (0.54)\\
$t=1.25$ &\bftab 3&\bftab 0.614&\bftab 0.005 (0.01) &\bftab [0.20 (0.43), 0.50 (0.37), 0.30 (0.11)]      &\bftab [10.51 (1.74), 5.26 (0.93), -0.03 (0.52)] & \bftab 10.50 (1.60) &\bftab -6.39 (1.03)\\
         &4       & 0.018      &  0.068 (0.04)      &[0.19 (0.31), 0.40 (1.41), 0.20 (1.33), 0.21 (0.74)]&[13.57 (3.51), 7.25 (2.12), 2.65 (2.55), -1.49 (1.25)] & 12.93 (2.53) & -7.96 (1.55)\\
         
\midrule

         &2       & 0.574      & 0.008 (0.02)       &[0.63 (1.61), 0.37 (1.61)]                        &[4.93 (1.10), 0.39 (0.84)] & 7.29 (0.78) & -4.35 (0.53) \\
$t=1.50$ &\bftab 3&\bftab 0.420&\bftab 0.007 (0.02) & \bftab [0.20 (0.27), 0.49 (0.29), 0.30 (0.19)]    & \bftab [10.44 (1.52), 5.23 (0.77), -0.09 (0.48)] & \bftab 10.38 (1.31) &\bftab -6.30 (0.84)\\
         &4       & 0.006      & 0.110 (0.07)       &[0.20 (0.00), 0.37 (0.94), 0.20 (0.00), 0.23 (0.94)]&[11.63 (1.32), 6.70 (0.35), 3.05 (3.10), -1.96 (2.20)] & 12.05 (1.12) & -7.24 (0.69)\\
         
\midrule 
\midrule   

TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \;]$  &   $[\; 10, \;5, \; 0 \;] $  &   $10$  &     $-6$           \\
\vspace{-0.35cm}

==> tables/Sim_Bin_slope2.tex <==
\label{tab_Ber_sl2}
        &  N clusters  & Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)    & $\hat{\beta}_1$(sd)  &  $\hat{\beta}_2$(sd)&    $\hat{\beta}_3$(sd)\\
                %ran_var = FALSE, ran_int = TRUE
\midrule
\midrule  

         &2&  & &   &  &  &    &    \\
$t=0.50$ &\bftab 3&n &n& n & n& n&   n&   n\\
         &4&  & &   &  &  &    &    \\
\midrule  
         &2&  & &   &  &  &    &    \\
$t=0.75$ &\bftab 3&n &n& n & n& n&   n&   n\\
         &4&  & &   &  &  &    &    \\
         
\midrule  
         &2&  & &   &  &  &    &    \\
$t=1.00$    &\bftab 3&n &n& n & n& n&   n&   n\\
         &4&  & &   &  &  &    &    \\

\midrule  
           &2&  & &   &  &  &    &    \\
$t=1.25$   &\bftab 3&n &n& n & n& n&   n&   n\\
           &4&  & &   &  &  &    &    \\
\midrule  
           &2&  & &   &  &  &    &    \\
$t=1.50$   &\bftab 3&n &n& n & n& n&   n&   n\\
           &4&  & &   &  &  &    &    \\           
\midrule               
\midrule 

              &2&  & &   &  &  &    &    \\
$\alpha=0.01$ &\bftab 3&n &n& n & n& n&   n&   n\\
              &4&  & &   &  &  &    &    \\
         
\midrule  
              &2&  & &   &  &  &    &    \\
$\alpha=0.05$ &\bftab 3&n &n& n & n& n&   n&   n\\
              &4&  & &   &  &  &    &    \\

\midrule  
              &2&  & &   &  &  &    &    \\
$\alpha=0.10$  &\bftab 3&n &n& n & n& n&   n&   n\\
              &4&  & &   &  &  &    &    \\


\midrule               
\midrule 
 

TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \;]$  &   $[\; 10, \;5, \; 0 \;] $  &   $10$  &   &   $-6$          &    $3$            \\
\vspace{-0.35cm}

==> tables/Sim_Poi_int.tex <==
\label{tab_Poi_int}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)     &   $\hat{\beta}_1$(sd)\\
             
\midrule
\midrule  

              &2        & 0.012        & 0.000 (0.00)   & [0.50 (0.00), 0.30 (0.00)]                           &  [1.01 (0.02), -0.98 (0.10)] & 0.29 (0.03)\\
$\alpha=0.01$ &\bftab 3 & \bftab 0.986 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.10)] & \bftab0.30 (0.02)   \\
              &4        & 0.002        & 0.000 (-)      & [0.20 (0.00), 0.50 (0.00), 0.10 (0.00), 0.20 (0.00)] &  [2.51 (-), 0.98 (-), -0.66 (-), -1.47 (-)] & 0.30 (-)  \\

\midrule  

              &2        & 0.018        & 0.000 (0.00)  & [0.50 (0.00), 0.30 (0.00)]                           & [1.00 (0.04), -0.98 (0.11)] & 0.30 (0.03)\\
$\alpha=0.05$ &\bftab 3 & \bftab 0.948 &\bftab 0.000 (0.00)  & \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]  &  \bftab [2.50 (0.02), 1.00 (0.03), -0.99 (0.10)] & \bftab0.30 (0.02)   \\
              &4        & 0.024        & 0.029 (0.03) & [0.20 (0.00), 0.38 (1.3), 0.19 (0.86), 0.23 (0.85)] & [2.51 (0.02), 1.06 (0.05), 0.19 (0.86), -1.20 (0.28)]& 0.29 (0.02)  \\
         

\midrule  
              &2        & 0.018        & 0.000 (0.00)        & [0.50 (0.00), 0.30 (0.00)]                            & [1.00 (0.03), -1.11 (0.13)] & 0.31 (0.02)\\
$\alpha=0.10$ &\bftab 3 & \bftab 0.872 & \bftab0.000 (0.00)  & \bftab[0.20 (0.10), 0.50 (0.19), 0.30 (0.00)]         &  \bftab [2.50 (0.07), 1.00 (0.03), -1.00 (0.10)] & \bftab0.30 (0.02)   \\
              &4        & 0.094        & 0.047 (0.04)       & [0.20 (0.20), 0.35 (1.57), 0.22 (1.15), 0.23 (0.83)]  &  [2.50 (0.03), 1.11 (0.29), 0.21 (0.84), -1.13 (0.23)]& 0.30 (0.02)  \\
\midrule              
\midrule      

         &2        & -       & -   & -                         &  - & -\\
$t=0.25$ &\bftab 3 & \bftab 0.846 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.10)] & \bftab0.30 (0.02)   \\
         &4        & 0.154        & 0.064 (0.04)      & [0.20 (0.00), 0.50 (0.00), 0.16 (0.48), 0.14 (0.48)] &  [2.49 (0.02), 1.00 (0.03), -0.87 (0.11), -1.30 (0.16)] & 0.30 (0.02)  \\
\midrule  

         &2        & 0.028        & 0.000 (0.00)   & [0.60 (0.93), 0.30 (0.00)]                           &  [1.36 (0.34), -0.97 (0.12)] & 0.30 (0.02)\\
$t=0.50$ &\bftab 3 & \bftab 0.950 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.10)] & \bftab0.30 (0.02)   \\
         &4        & 0.022        & 0.014 (0.01)      & [0.20 (0.00), 0.50 (0.00), 0.15 (0.50), 0.15 (0.50)] &  [2.51 (0.02), 1.00 (0.02), -0.77 (0.18), -1.39 (0.21)] & 0.31 (0.02)  \\
\midrule  


         &2        & 0.066        & 0.000 (0.00)   & [0.58 (1.34), 0.33 (1.19)]                           &  [1.43 (0.42), -0.90 (0.42)] & 0.31 (0.03)\\
$t=0.75$ &\bftab 3 & \bftab 0.934 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.10)] & \bftab0.30 (0.02)   \\
         &4        & -        & -      & - &  - & -  \\
\midrule  

         &2        & 0.110        & 0.000 (0.00)   & [0.61 (1.33), 0.33 (1.14)]                           &  [1.50 (0.39), -0.94 (0.40)] & 0.30 (0.04)\\
$t=1.00$ &\bftab 3 & \bftab 0.890 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.10)] & \bftab0.30 (0.02)   \\
         &4        & -        & -      & - &  - & -  \\

\midrule  

         &2        & 0.296        & 0.000 (0.00)   & [0.50 (2.16), 0.46 (2.31)]                           &  [1.79 (0.55), -0.50 (0.76)] & 0.30 (0.03)\\
$t=1.25$ &\bftab 3 & \bftab 0.704 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]     &  \bftab [2.50 (0.02), 1.00 (0.03), -1.00 (0.09)] & \bftab0.30 (0.02)   \\
         &4        & -        & -      & - &  - & -  \\


\midrule  

%         &2        & 0.734        & 0.000 (0.00)   &        [0.59 (1.77), 0.37 (1.78)]                 &  [1.71 (0.39), -0.77 (0.58)] & 0.30 (0.04)\\
%$t=1.50$ &\bftab 3 & \bftab 0.266 & \bftab0.000 (0.00)& \bftab[0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]  &  \bftab [2.51 (0.02), 0.98 (0.02), -1.02 (0.09)] & \bftab0.30 (0.02)   \\
%         &4        & -        & -      & - &  - & -  \\
        

\midrule                 
\midrule  

TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \; ]$  &   $[\; 2.5, \; 1,\; -1 \;]$          &   $0.3$              \\
\vspace{-0.35cm}

==> tables/Sim_Poi_int2.tex <==
\label{tab_Poi_int2}
        &  N clusters  &Proportion (out of 500) & Entropy(sd)&   $\hat{\omega}$(sd) & $\hat{c}_1$(sd)     &   $\hat{\beta}_1$(sd)&    $\hat{\beta}_2$(sd)\\


\midrule                
\midrule 

              &2       & 0.040        &0.000 (0.00)& [0.50 (0.00), 0.30 (0.00)]  & [0.99 (0.04), -0.99 (0.14)] & 0.29 (0.02) & 0.90 (0.03)\\
$\alpha=0.01$ &\bftab 3& \bftab 0.956 &\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)] & \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.08)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02)\\
              &4       & 0.004        &0.006 (0.00)&  [0.20 (0.00), 0.20 (0.00), 0.30 (0.00), 0.30 (0.00)] & [2.52 (0.00), 1.14 (0.00), 0.94 (0.00), -1.02 (0.00)] & 0.33 (0.00) & 0.88 (0.00)\\
         
\midrule   
              &2       &0.028       &0.000 (0.00)& [0.50 (0.00), 0.30 (0.00)]   & [1.00 (0.02), -1.06 (0.09)] & 0.31 (0.02) & 0.90 (0.02)\\
$\alpha=0.05$ &\bftab 3&\bftab 0.934&\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)] & \bftab [2.50 (0.02), 1.00 (0.03), -1.00 (0.08)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02) \\
              &4       &0.036       &0.015 (0.02)&  [0.19 (0.31), 0.37 (1.76), 0.24 (1.34), 0.21 (0.85)]  &[2.50 (0.02), 1.18 (0.45), -0.11 (0.88), -1.26 (0.26)] & 0.30 (0.01) & 0.90 (0.01)\\
         
\midrule  
              &2       &0.028       & 0.000 (0.00) & [0.50 (0.00), 0.30 (0.00)]  & [0.99 (0.02), -0.95 (0.06)] & 0.30 (0.01) & 0.91 (0.02)\\
$\alpha=0.10$ &\bftab 3&\bftab 0.870& \bftab 0.000 (0.00) & \bftab [0.20 (0.21), 0.50 (0.31), 0.30 (0.07)] & \bftab [2.49 (0.12), 0.99 (0.12), -0.99 (0.09)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02)\\
              &4       &0.098       & 0.043 (0.04) & [0.19 (0.27), 0.35 (1.40), 0.20 (1.25), 0.26 (0.64)]  &[2.50 (0.03), 1.16 (0.40), 0.38 (0.80), -1.08 (0.14)] & 0.30 (0.02) & 0.90 (0.01)\\
              
\midrule
\midrule  	

         &2       & 0.024      & 0.000 (0.00)  & [0.51 (0.28), 0.30 (0.00)] &[1.02 (0.13), -1.00 (0.10)] & 0.30 (0.01) & 0.89 (0.04) \\
$t=0.50$ &\bftab 3&\bftab 0.968&\bftab 0.000 (0.00)& \bftab [0.20 (0.14), 0.50 (0.18), 0.30 (0.05)] &\bftab [2.50 (0.07), 1.00 (0.08), -1.00 (0.09)] & \bftab 0.30 (0.02) & \bftab 0.90 (0.02)\\
         &4       & 0.008      & 0.000 (0.00) &  [0.20 (0.00), 0.50 (0.00), 0.20 (0.00), 0.10 (0.00)] &[2.50 (0.01), 1.00 (0.02), -0.84 (0.02), -1.41 (0.03)] & 0.30 (0.02) & 0.90 (0.01)\\
\midrule  
         &2       &0.088        & 0.000 (0.00)& [0.50 (1.71), 0.40 (2.0)]  &[1.28 (0.39), -0.91 (0.35)] & 0.29 (0.04) & 0.86 (0.05) \\
$t=0.75$ &\bftab 3&\bftab 0.912 &\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)] & \bftab [2.50 (0.02), 1.00 (0.03), -1.00 (0.09)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02)\\
         &4       &  -          & - & -  & - & - &   - \\
         
\midrule  
         &2       & 0.172      & 0.000 (0.00) & [0.56 (1.19), 0.32 (1.05)]  & [1.35 (0.42), -0.91 (0.35)] & 0.29 (0.04) & 0.86 (0.05)\\
$t=1.00$ &\bftab 3&\bftab 0.828&\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)]  & \bftab [2.50 (0.02), 1.00 (0.03), -1.01 (0.08)] & \bftab 0.30 (0.02) & 0.90 (0.02) n\\
         &4       &  -          & - & -  & - & - &   - \\

\midrule  
         &2       &  0.340     &0.000 (0.00) & [0.50 (1.71), 0.40 (2.00)]  & [1.52 (0.57), -0.64 (0.64)] & 0.30 (0.03) & 0.88 (0.05) \\
$t=1.25$ &\bftab 3&\bftab 0.660&\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)] & \bftab [2.50 (0.02), 1.01 (0.03), -1.00 (0.08)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02)\\
         &4       &  -          & - & -  & - & - &   - \\
           
\midrule  
         &2       & 0.808       & 0.000 (0.00)& [0.51 (1.64), 0.39 (1.89)]  & [1.52 (0.54), -0.67 (0.61)] & 0.29 (0.04) & 0.87 (0.05)\\
$t=1.50$ &\bftab 3&\bftab 0.192 &\bftab 0.000 (0.00)& \bftab [0.20 (0.00), 0.50 (0.00), 0.30 (0.00)] & \bftab [2.51 (0.02), 0.99 (0.02), -1.01 (0.09)] & \bftab 0.30 (0.01) & \bftab 0.90 (0.02)\\
         &4       &  -          & - & -  & - & - &   -  \\
         

\midrule               
\midrule  

TV       & &     &  & $[\; 0.2, \; 0.5, \; 0.3 \; ]$  &   $[\; 2.5, \; 1,\; -1 \;]$          &   $0.3$          &    $0.9$            \\
\vspace{-0.35cm}
